Reliable a-posteriori error estimators for $hp$-adaptive finite element approximations of eigenvalue/eigenvector problems

We present reliable a-posteriori error estimates for $hp$-adaptive finite element approximations of eigenvalue/eigenvector problems. Starting from our earlier work on $h$ adaptive finite element approximations we show a way to obtain reliable and efficient a-posteriori estimates in the $hp$-setting. At the core of our analysis is the reduction of the problem on the analysis of the associated boundary value problem. We start from the analysis of Wohlmuth and Melenk and combine this with our a-posteriori estimation framework to obtain eigenvalue/eigenvector approximation bounds.

==> appendA.tex <==
This discussion is taken over from \cite[Proposition 3.2]{GrubisicTKpp} and we repeat it since it
has only been published before as an arxiv preprint. In what follows we need the block diagonal part of the operator $A$.
It is the self-adjoint operator $\mH_P$ which is defined in the sense of Kato by the form $B_P(\cdot,\cdot)=B(P\cdot, P\cdot)+
B(P_\perp\cdot,P_\perp\cdot)$. Here we use $P$ to denote the orthogonal projection onto the space $\hat S_m$ and $P_\perp=I-P$.
Let us examine $\eta_i$ in  further detail we have
\begin{equation}\label{eq.sing_val_2}
\eta_i(P):=\Big[\max_{\substack{\mathcal{S}\subset\ra(P),\\
\dim(\mathcal{S})=m-i+1}}\min\big\{\frac{(\psi,
\mH^{-1}\psi)-(\psi,\mH^{-1}_P\psi)}{(\psi,\mH^{-1}\psi)}~
\big|~\psi\in\mathcal{S}, \|\psi\|=1\big\}\Big]^{1/2},
\end{equation}
for $i=1, \ldots, m$. Before we turn to the main theorem,
let us give an alternative---more common---definition for the approximation defects $\eta_i(P)$.
To this end we further exploit the Galerkin orthogonality
property of the $P$-diagonal part of $h$ and in particular the ramifications of
relation (\ref{eq:galerkinB}). For any
$f\in\ra(P)$ we have
$$
B[\mH^{-1}
f-\mH^{-1}_Pf]=\Big[\sup_{\phi\in\q(B)\setminus\{0\}}\frac{|B(\mH^{-1}
f-\mH^{-1}_Pf,\phi)|}{h[\phi]^{1/2}}\Big]^{2}=\|\mH\Xi^{-1}
f-f\|_{\mH^{-1}}^2.
$$
With this
we can write (\ref{eq.sing_val_2}) in an
alternative form
\begin{equation}\label{eq.sing_val_3}
\eta_i(P):=\Big[\max_{\substack{\mathcal{S}\subset\ra(P),\\
\dim(\mathcal{S})=m-i+1}}\min\big\{\frac{\|\mH
\Xi^{-1}\psi-\psi\|_{\mH^ {-1}}^2}{\|\psi\|_{\mH^ {-1}}^2}~
\big|~\psi\in\mathcal{S}, \|\psi\|=1\big\}\Big]^{1/2},
\end{equation}
for $i=1, \ldots, m$.

We only explicitly present arguments that $\eta_m(P)<1$.
This fact was first established, in the matrix case, by Z. Drma\v{c},
Zagreb. Since $\ra(P)$ reduces $\mH_P$ we have
$$
B(\mH^{-1}_{P} f,v)=h_{P}(\mH^{-1}_{P} f,v)=(f,v),\qquad v\in\ra(P),
$$
i.e. $\mH^{-1}_{P}f$ is a Galerkin approximation from the subspace
$\ra(P)$ to $\psi=\mH^{-1}f$, which solves the problem $\mH\psi=f$.
With this in hand one computes
\begin{equation}\label{eq:galerkinB}
B(\mH^{-1} f-\mH^{-1}_{P} f,\mH^{-1} g-\mH^{-1}_{P}
g)=(f,\mH^{-1}g)-(f,\mH^{-1}_{P}g), \qquad f,g\in\ra(P).
\end{equation}
This implies
$(f,\mH^{-1}f)\geq(f,\mH_P^{-1}f)\geq 0$, $f\in\ra(P)$ and $0\leq\eta_i(P)\leq 1$ follows.
Assume $\eta_m(P)=1$, then there exists
$f\in\ra(P)\setminus\{0\}$ such that $(f,\mH^{-1}_Pf)=0$.
This is an obvious contradiction with the fact that $\mH_P$ is
positive definite.

Now, set formally $\lambda_0(\mH):=0$, $\fG_0:=\infty$ and define
\begin{align}\fG_q&:=\min\Big\{
|\lambda_{q}(\mH)-\mu|\mu^{-1}:\mu\in\spec(\mH_P)\setminus\{\mu_1,...,\mu_m\}\Big\}\\
\gamma_s(\lambda_q)&:=\min\Big\{
\frac{\lambda_{q+m}(\mH)-\mu_m}{\lambda_{q+m}(\mH)+\mu_m},
\frac{\mu_1-\lambda_{q-1}(\mH)}{\mu_1+\lambda_{q-1}(\mH)}\Big\},\label{eq.uvijet123}
\end{align}
for $q\in\N$. This quantities---which measure the sensitivity of the eigenvalue $\lambda_q(\mH)$---will play a role in the
statement of the theorems in the next section. In the rest of the section we suppress the dependence of quantities
on $\mH$ and $P$ in the notation.


\begin{proposition}\label{prop:lower}
Let $\lambda_m<\lambda_{m+1}$ and let $\ra(P)$, $\dim\ra(P)=m$ be the test space for the form $h$ such that $2\eta_m<1$ then
$$
\frac{1\mu_1}{2\mu_m}\sum_{i=1}^m \frac{\|\mH u_i-\mu_i
u_i\|^2_{\mH^{-1}}}{\|\mH u_i\|^2_{\mH^{-1}}}\leq
\sum^m_{i=1}\frac{\mu_i-\lambda_i}{\mu_i}.
$$
\end{proposition}
\begin{proof}
Let $u_i\in\ra(P)$, $i=1,...,m$ be the Ritz vectors. The proof follows from
\begin{align*}
\sum^m_{i=1}\|\mH \frac{1}{\mu_i}u_i-u_i\|^2_{\mH^{-1}}&=\sum^m_{i=1}\Big[(u_i,\mH^{-1}u_i)-(u_i,\Xi^{-1}u_i)\Big]
=\sum^m_{i=1}\Big[(u_i,\mH^{-1}u_i)-\frac{1}{\mu_i}\Big]\\
&\leq\sum^m_{i=1}\Big[\frac{1}{\lambda_i}-\frac{1}{\mu_i}\Big]=\sum^m_{i=1}\frac{\mu_i-\lambda_i}{\lambda_i\mu_i}.
\end{align*}
 Note that according to (\ref{eq:Diag}) below, we have
$\sum_{i=1}^m\eta^2_i \leq \sum_{i=1}^m
\frac{\|\mH u_i-\mu_i u_i\|^2_{\mH^{-1}}}{\|\mH u_i\|^2_{\mH^{-1}}}$.
\end{proof}

==> exper_oct12.tex <==
In the numerical experiments we illustrate the efficiency of the estimator (\ref{relyhp}) by considering several model problems for which we have
explicit formula for the eigenvalues available.

We plot the effectivity quotient
$$
\frac{\sum^\textsc{m}_{i=1}\!
  \frac{\hat\lambda_i-\lambda_i}
  {\hat\lambda_i}}{\sum_{i=1}^\textsc{m}\hat\lambda_i^{-1}\varepsilon_i^2}
$$
against the $\text{dim}(V^p_k)$ for several of the model problems from \cite{GiGrOv}.

\subsection{Laplacian on the Unit Square}\label{sub1}
We illustrate some of the basic features of our approach, and
introduce terminology used for other experiments, on the following
simple problem: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1_0(\Omega)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega\ , \\
u&=\ 0\ , & \mbox{on }\partial\Omega \ .
\end{array}
\right.
\end{equation}


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_laplace_h.eps}
\end{center}
\caption{\label{fig:lap_err} Errors and a posteriori estimations for different values of $p$}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_laplace_h.eps}
\end{center}
\caption{\label{fig:lap_rel} Effectivity index for different values of $p$}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_laplace_hp.eps}
\end{center}
\caption{\label{fig:lap_err_hp} Errors and a posteriori estimations using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_laplace_hp.eps}
\end{center}
\caption{\label{fig:lap_rel_hp} Effectivity index for different values using the $hp$-adaptivity}
\end{figure}

Here, $\Omega=(0,1)^2$ is the unit square.  Because the eigenvalues
and eigenfunctions (which are analytic) are known explicitly,
$\lambda_{ij}=(i^2+j^2)\pi$ and $u_{ij}=\sin(i\pi x)\sin(j\pi y)$, it
is trivial to check certain properties of our estimator and adaptive
scheme.  This indicates how our approach might be expected to perform
in such ideal cases --- although we will see that similar performance is
achieved in low-regularity situations as well.

In Figure~\ref{fig:lap_err} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ for different values of $p$ and using $h-$adaptivity only. The slopes of the curves are in agreement with the theory.
In Figure~\ref{fig:lap_rel} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err}.
As can be seen the values of $C$ are very well clustered, as predicted by the theory.
Moreover, in Figure~\ref{fig:lap_err_hp} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_hp} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err_hp}, again the values of $C$ are very well clustered, as predicted by the theory.

\subsection{Laplacian on the Unit Square with Neumann Boundary
  Conditions}\label{sub2}

\begin{quote}
  What is our interest in the Neumann problem?  I do not necessarily
  object to having it, but I do not see why we have both the Dirichlet
  and Neumann problems for the unit square. \hfill Jeff
\end{quote}

\begin{quote}
  I started to work on Neumann problems to beef up the numeric section and to test the code. Anyway anything that we are removing from this paper, could be used in the Ilas paper.
  Since pure Neumann problems are not in the scope of the paper, I agree to remove them. \hfill Stefano
\end{quote}

Now we consider the a modification of the previous example: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1(\Omega)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap_neum}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega\ , \\
\nabla u\cdot n&=\ 0\ , & \mbox{on }\partial\Omega \ .
\end{array}
\right.
\end{equation}


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_laplace_neu_hp.eps}
\end{center}
\caption{\label{fig:lap_err_neu_hp} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_laplace_neu_hp.eps}
\end{center}
\caption{\label{fig:lap_rel_neu_hp} Effectivity index using the $hp$-adaptivity}
\end{figure}

Here, $\Omega=(0,1)^2$ is the unit square.  Because the eigenvalues
and eigenfunctions (which are analytic) are known explicitly,
$\lambda_{ij}=((i-1)^2+(j-1)^2)\pi$ and $u_{ij}=\cos(i\pi x)\cos(j\pi y)$.

Moreover, in Figure~\ref{fig:lap_err_neu_hp} we plot the error $\sum_{i=2}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=2}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity, we haven't considered the first eigenvalue because $\lambda_1=0$. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_neu_hp} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err_neu_hp}, again the values of $C$ are very well clustered, as predicted by the theory.

\subsection{Eigenvalues with Discontinuous Potential}
\begin{quote}
I assume here that we are using highly-accurate eigenvalue
approximations to compute ``exact'' errors in this case, but correct
me if I'm wrong.  It is interesting to me that the third eigenfunction
is the problem in this case.  Is it possible to put in contour plots
of the computed eigenvalues for now? Even though they may not be in the
submitted version, I would like to see how they look.  All of them
should be at least in $H^2$, but I am not sure what to expect of their
behavior near the interfaces and crosspoint. \hfill Jeff
\end{quote}

\begin{quote}
Yes, I used highly-accurate eigenvalue
approximations for reference values.
 \hfill Stefano
\end{quote}

We consider the family of problems on the domain $[-1,1]^2$, such that
%\begin{equation}\label{eq:dauge}
%\left\{
%\begin{array}{rlr}\
%-\triangle u+\kappa V_{MD}\cdot\psi=\lambda u,& \mbox{in }\Omega\ , \\
%\nabla u\cdot n&=\ 0\ , & \mbox{on }\partial\Omega \ .
%\end{array}
%\right.
%\end{equation}
\begin{align}\label{eq:dauge}
\left\{
\begin{array}{ll}\
-\triangle u+\kappa V_{MD}\cdot\psi=\lambda u& \mbox{in }\Omega\ , \\
\nabla u\cdot n=\ 0\  & \mbox{on }\partial\Omega \ .
\end{array}
\right.
\end{align}
%\begin{align}\label{eq:dauge}
%&-\triangle\psi+\kappa V_{MD}\cdot\psi=\lambda\psi,\\ &\psi\in H^1_0([-1,1]^2), \|\psi\|_{0}=1.
%\end{align}
where the function $V_{MD}$ is defined as the characteristic function
of the coalescent squares which are denoted by $\mathcal{M}_1$ in
Figure \ref{figMonique}.
%This example was originally proposed and
%solved as a test example for an eigenvalue problem in electromagnetism by
%M. Dauge in \cite{DaugeW}. In its original formulation the problem is much more challenging, since
%the jumps are contained in the second order term, cf. \cite{DaugeW}. A similar problem --- having jumps in the second order term --- has also been
%studied as an interesting example in the context of ill-posed boundary value problems by Knyazev and Widlund in \cite{Knyazev2003}. There,
%an extensive regularity theory for such problems is presented as well.


\begin{figure}[h!]
\begin{center}
%\includegraphics[width=8.5cm]{2DomE.eps}
\begin{picture}(0,0)%
\includegraphics{Dauge.eps}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2724,2724)(1339,-523)
\put(1850,1490){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_2$}%
}}}}
\put(3200,140){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_2$}%
}}}}
\put(3200,1490){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_1$}%
}}}}
\put(1850,140){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_1$}%
}}}}
\end{picture}%
\end{center}
\caption{\label{figMonique} A modification of the touching squares example of M. Dauge. The potential $V_{MD}$ is the characteristic
function of the coalescent squares denoted by $\mathcal{M}_1$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_neu_jumps_0.5.eps}
\end{center}
\caption{\label{fig:error_neu_jumps_0.5} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_neu_jumps_0.5.eps}
\end{center}
\caption{\label{fig:rel_neu_jumps_0.5} Effectivity index using the $hp$-adaptivity}
\end{figure}


As first example we choose $\kappa=0.5$.
In Figure~\ref{fig:error_neu_jumps_0.5} we plot the error $\sum_{i=2}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=2}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity, also in Figure~\ref{fig:rel_neu_jumps_0.5} we plot the correspondent values of the effectivity constant $C$.
As can be seen the convergence is quite fast.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_neu_jumps_eig1.eps}
\end{center}
\caption{\label{fig:error_neu_jumps_eig1} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_neu_jumps_eig1.eps}
\end{center}
\caption{\label{fig:rel_neu_jumps_eig1} Effectivity index using the $hp$-adaptivity}
\end{figure}


Then we choose $\kappa=0.1$ and we consider the first eigenvalue different from zero.
In Figure~\ref{fig:error_neu_jumps_eig1} we plot the error $\frac{\hat\lambda_2-\lambda_2}{\hat\lambda_2}$ and the residuals ${\hat\lambda_2}^{-1}\varepsilon_2^2$ using $hp-$adaptivity, also in Figure~\ref{fig:rel_neu_jumps_eig1} we plot the correspondent values of the effectivity constant $C$.

It is interesting to compare the previous plots with the next ones, where we consider the first three eigenvalues different from 0, namely $\lambda_j$, $j=2,3,4$.
In Figure~\ref{fig:error_neu_jumps_0.1} we plot the error and the residuals and in Figure~\ref{fig:rel_neu_jumps_0.1} we plot the correspondent values of the effectivity constant $C$.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_neu_jumps_0.1.eps}
\end{center}
\caption{\label{fig:error_neu_jumps_0.1} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_neu_jumps_0.1.eps}
\end{center}
\caption{\label{fig:rel_neu_jumps_0.1} Effectivity index using the $hp$-adaptivity}
\end{figure}

As can be seen the convergence is much slower and the reason for that can be found looking at Figure~\ref{fig:error_split_neu_jumps_0.1} where we plot the errors for each eigenvalue separately.
As can be seen it is the third eigenvalue that is the slowest and the one to slow down the overall convergence. This seems to suggest that the third eigenvalue is much less regular than the other two.
In Figure~\ref{fig:eig2},~\ref{fig:eig3} and~\ref{fig:eig4} we plot the counter plots for the three considered eigenfunctions.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_neu_jumps_0.1.eps}
\end{center}
\caption{\label{fig:error_split_neu_jumps_0.1} Errors from each eigenvlaue}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0002.eps}
\end{center}
\caption{\label{fig:eig2} Second eigenfunction.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0003.eps}
\end{center}
\caption{\label{fig:eig3} Third eigenfunction.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0004.eps}
\end{center}
\caption{\label{fig:eig4} Fourth eigenfunction.}
\end{figure}

\subsection{Laplacian on a Triangular Domain}
\begin{quote}
  Again, I do not object to this problem, but I am not sure what our
  interest is.  Unless I have read \cite{McCartin2003} incorrectly,
  the eigenvalues for this problem should be
\[
\lambda_{mn}=\frac{16\pi^2}{9}(m^2+mn+n^2)~,
\]
and explicit expressions are also given for the eigenfunctions.  We
could use these for the computation error analysis.  Since these are
less well-known than those for rectangular or elliptic regions, they
might be of interest to some; but they are not ``hard'' problems in
the sense singularities or near-singularities.  I have included this
paper in the DropBox folder.
If we want to go this route, we McCartin has a few more papers in this
series where he considers other types of boundary conditions:
\cite{McCartin2002,McCartin2007,McCartin2008}.  I do not have copies
of the most recent two. \hfill Jeff
\end{quote}

\begin{quote}
I have computed this problem in preparation for the two problems on a triangle with a hole, see below.
 \hfill Stefano
\end{quote}

We now look for the eigenvalues of the problem: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1_0(\Omega)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega\ , \\
u&=\ 0\ , & \mbox{on }\partial\Omega \ .
\end{array}
\right.
\end{equation}
where $\Omega$ is a equilateral triangle with unit edge.
The exact values of the eigenvalues for this problem are given by:
\[
\lambda_{mn}=\frac{16\pi^2}{9}(m^2+mn+n^2)~,
\]
which is presented in \cite{McCartin2003}.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_tri.eps}
\end{center}
\caption{\label{fig:error_tri} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_tri.eps}
\end{center}
\caption{\label{fig:rel_tri} Effectivity index using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_tri.eps}
\end{center}
\caption{\label{fig:error_split_tri} Errors from each eigenvlaue}
\end{figure}


In Figure~\ref{fig:error_tri} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In this case the convergence is exponential and in Figure~\ref{fig:rel_tri} we plot the values of the effectivity constant $C$. For this example, it is interesting to notice that all the considered eigenvalues converge at the same speed, as can be seen in Figure~\ref{fig:error_split_tri} where the error for each eigenvalue is plot separately.

\subsection{Laplacian on the Unit Square with a Hole}


The next problem we present is defined on the domain $\Omega:=[0,1]^2/ [1/3,2/3]^2 $: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1_0(\Omega)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap_sq_hole}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega\ , \\
u &=\ 0\ , & \mbox{on }\partial\Omega \ .
\end{array}
\right.
\end{equation}


\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_laplace_hole_hp.eps}
\end{center}
\caption{\label{fig:lap_err_hole_hp} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_laplace_hole_hp.eps}
\end{center}
\caption{\label{fig:lap_rel_hole_hp} Effectivity index using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_laplace_hole_hp.eps}
\end{center}
\caption{\label{fig:lap_err_split_hole_hp} Errors from each eigenvlaue}
\end{figure}



Moreover, in Figure~\ref{fig:lap_err_hole_hp} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_hole_hp} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err_hole_hp}, again the values of $C$ are very well clustered, as predicted by the theory. Finally, in Figure~\ref{fig:lap_err_split_hole_hp} there are the plots of the error for each eigenvalue separately.

\subsection{Laplacian on a Triangular Domain with on a Hole}

We now look for the eigenvalues of the problem: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1_0(\Omega_i)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap_triang_hole}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega_i\ , \\
u&=\ 0\ , & \mbox{on }\partial\Omega_i \ .
\end{array}
\right.
\end{equation}
where $\Omega_i$ is an equilateral triangle with unit edge with either with an equilateral triangle hole of edge 1/4 pointing either up ($\Omega_1$) or down ($\Omega_2$);



\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_triup.eps}
\end{center}
\caption{\label{fig:error_triup} Errors and a posteriori estimation using the $hp$-adaptivity for $\Omega_1$}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_tridown.eps}
\end{center}
\caption{\label{fig:error_tridown} Errors and a posteriori estimation using the $hp$-adaptivity for $\Omega_2$}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_triup.eps}
\end{center}
\caption{\label{fig:rel_triup} Effectivity index using the $hp$-adaptivity for $\Omega_1$}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_tridown.eps}
\end{center}
\caption{\label{fig:rel_tridown} Effectivity index using the $hp$-adaptivity for $\Omega_2$}
\end{figure}



In Figures~\ref{fig:error_triup} and~\ref{fig:error_tridown} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity for each domain, and in Figures~\ref{fig:rel_triup} and~\ref{fig:rel_tridown} we plot the values of the effectivity constant $C$.

\subsection{Eigenvalues on a Slit Unit Suare}

We now consider the unit square domain $[0,1]^2$ with a slit $S$ from $(0.5,0.5)$ to $(1,0.5)$: {\it Find eigenpairs $(\lambda,u)\in \mathbb{R}\times
  H^1(\Omega)$ such that $\|u\|_{0}=1$, where}
\begin{equation}\label{eq:lap_slit_square}
\left\{
\begin{array}{rlr}\
-\triangle u&=\ \lambda u,& \mbox{in }\Omega\ , \\
u&=\ 0\ , & \mbox{on }\partial\Omega \ , \\
\nabla u\cdot n&=\ 0\ , & \mbox{on }S \ .
\end{array}
\right.
\end{equation}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_crack2.eps}
\end{center}
\caption{\label{fig:lap_err_crack2_hp} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_crack2.eps}
\end{center}
\caption{\label{fig:lap_rel_crack2_hp} Effectivity index using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_crack.eps}
\end{center}
\caption{\label{fig:lap_err_crack_hp} Errors and a posteriori estimation using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_crack2.eps}
\end{center}
\caption{\label{fig:lap_rel_crack_hp} Effectivity index using the $hp$-adaptivity}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_crack.eps}
\end{center}
\caption{\label{fig:lap_err_split_crack_hp} Errors from each eigenvlaue}
\end{figure}


We start considering the second eigenvalue, which seems to be highly irregular.
In Figure~\ref{fig:lap_err_crack2_hp} we plot the error $\frac{\hat\lambda_2-\lambda_2}{\hat\lambda_2}$ and the residuals ${\hat\lambda_2}^{-1}\varepsilon_2^2$ using $hp-$adaptivity. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_crack2_hp} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err_crack2_hp}, again the values of $C$ are very well clustered, as predicted by the theory. Then, in Figure~\ref{fig:lap_err_crack_hp} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_crack_hp} we plot the values of the effectivity constant $C$.
Comparing  Figure~\ref{fig:lap_err_crack2_hp} with Figure~\ref{fig:lap_err_crack_hp} it is clear that the convergence is very similar, but then looking at Figure~\ref{fig:lap_err_split_crack_hp}, where the plots of the error for each eigenvalue are reported, it is also clear that the error for the second eigenvalue is dominant compared to the errors for the other eigenvalues, which are smoother and converge faster.



\subsection{Eigenvalues on a Slit Disk}
\begin{quote}
Do you think that we will be able to do this kind of problem?
I am very interested, and think that others would be impressed
if we showed exponential convergence here.  Even the
change-of-variables itself might be of interest to some readers.
\hfill Jeff
\end{quote}

\begin{quote}
I'm going to spend more time on this problem, once I'm back in Nottingham.\hfill Stefano
\end{quote}

Let $\Omega$ be the unit disk with the non-negative $x$-axis
removed---described by the polar inequalities $0<r<1$,
$0<\theta<2\pi$.  We consider problem: Find
$\psi\neq 0$
and $\lambda$ such that
\begin{align}\label{slit_eig_prob}
-\Delta \psi=\lambda\psi\mbox{ in }\Omega\;,\;
\psi=0\mbox{ when }r=1\mbox{ or }\theta=0\;,\;\mbox{ and }
\frac{\partial \psi}{\partial\theta}=0\mbox{ when }\theta=2\pi~.
\end{align}
In words, homogeneous Dirichlet conditions are imposed on the boundary
of the disk and on the top of the slit, and homogeneous Neumann
conditions are imposed on the bottom of the slit.  Let
$\nu_k=(2k-3)/4$ for $k\in\NN$, and $z_{km}$ be the $m^{th}$ positive
root of the first-kind Bessel functions $J_{\nu_k}$.  It is
straightforward to verify that, up to (non-zero) scaling of
eigenfunctions, all solutions of~\eqref{slit_eig_prob} are given by
\begin{align*}
\lambda_{km}=z_{km}^2\quad,\quad
\psi_{km}=J_{\nu_k}(z_{km}r)\sin(\nu_k \theta)\quad,\quad k,m\in\NN~.
\end{align*}
We see that
$\psi_{km}\sim \sin(\nu_k
\theta)\left(\frac{z_{km}r}{2}\right)^{\nu_k}$ as $r\to 0$, so
singularities of types $r^{\nu_k}$ occur infinitely many times
in the spectrum.  The strongest of these singularities is of type
$r^{1/4}$, and it occurs in the eigenfunctions associated
with the first (smallest) and sixth eigenvalues, for example.
The eigenvalues can, in principle, be computed to abitrary precision
by using a computer algebra system, and we give
the smallest six of them below, accurate to all $30$ digits
shown---up to rounding in the last digit.
\begin{align*}
\begin{array}{|ccc|}
\hline
k&m&\lambda_{km}\\\hline
1&1&7.73333653346596686390263803337\\
2&1&12.1871394680951290047505723560\\
3&1&17.3507761313694859586686502730\\
4&1&23.1993865387331719385298116070\\
5&1&29.7145342842106938075714690649\\
1&2&34.8825215790904790430911907100\\\hline
\end{array}
\end{align*}
%%% 6&1&36.8818928841180487579063517659



==> exper_oct17.tex <==
In the numerical experiments we illustrate the efficiency of the
estimator (\ref{relyhp}) by considering several model problems for
which we have explicit formula for the eigenvalues available.  We
consider several problems of the general form
\begin{align}\label{gen_eig_prob}
\cL \psi=\lambda\psi\mbox{ in }\Omega\quad,\quad \|\psi\|=1~,
\end{align}
for a second-order, linear elliptic operator $\cL$, where homogeneous
Dirichlet or Neumann conditions are imposed on the boundary.  Plots
are given of the total relative error, its \textit{a posteriori}
estimate, and the associated effectivity quotient, shown,
respectively, below:
\begin{align*}
  \sum^\textsc{m}_{i=1}\!  \frac{\hat\lambda_i-\lambda_i}
  {\hat\lambda_i} \quad,\quad
  \sum_{i=1}^\textsc{m}\hat\lambda_i^{-1}\varepsilon_i^2 \quad,\quad
  \frac{\sum^\textsc{m}_{i=1}\!  \frac{\hat\lambda_i-\lambda_i}
    {\hat\lambda_i}}{\sum_{i=1}^\textsc{m}\hat\lambda_i^{-1}\varepsilon_i^2}~.
\end{align*}
These are plotted against the size of the discrete
problem $\text{dim}(V^p_k)$.  For most of our problems, the exact
eigenvalues are unknown, so we take highly accurate computations on
very large problems as ``exact'' for these comparisons.

\begin{figure}[h!]
\begin{center}
\includegraphics[height=2.0in]{TriangleHole.eps}
\includegraphics[width=2.0in]{SlitSquare.eps}
\includegraphics[width=2.0in]{SlitCircle.eps}
\end{center}
\caption{\label{fig:domains} Some of the domains used for the experiments.}
\end{figure}

\subsection{Dirichlet Laplacian on the Unit Triangle}\label{Triangle}
As a simple problem for which the eigenvalues and eigenfunctions are
explicitly known (cf.~\cite{McCartin2003}), we consider the problem
where: $\cL=-\Delta$, $\Omega$ is equilateral triangle of having
unit edge-length, and $\psi=0$ on $\partial\Omega$. The eigenvalues
can be indexed as
\[
\lambda_{mn}=\frac{16\pi^2}{9}(m^2+mn+n^2)~,
\]
and we refer interested readers to~\cite{McCartin2003} for explicit
descriptions of the eigenfunctions. 
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_tri.eps}
\end{center}
\caption{\label{fig:error_tri} Errors and error estimates. Triangle problem.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_tri.eps}
\end{center}
\caption{\label{fig:rel_tri} Effectivity index. Triangle problem.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_tri.eps}
\end{center}
\caption{\label{fig:error_split_tri} Errors from each
  eigenvlaue. Triangle problem.}
\end{figure}
In Figure~\ref{fig:error_tri} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In this case the convergence is exponential and in Figure~\ref{fig:rel_tri} we plot the values of the effectivity quotient. For this example, it is interesting to notice that all the considered eigenvalues converge at the same speed, as can be seen in Figure~\ref{fig:error_split_tri} where the error for each eigenvalue is plot separately.

\subsection{Dirichlet Laplacian on the Unit Triangle with on a
  Hole}\label{Triangle_Hole}
We now consider the problem where $\cL=-\Delta$, $\Omega$ is the
equaliteral unit triangle with an equilateral triangle having
edgelength $1/4$ removed from its center (see Figure~\ref{fig:domains}), and $\psi=0$ on
$\partial\Omega$.  For such a problem, it is expected that some of the
eigenfunctions will have an $r^{3/5}$-type singularity at each of the
three interior corners, where $r$ is the distance to the nearest
corner.  In this case, the exact eigenvalues are unknown.

In Figure~\ref{fig:error_triup} we plot
the relative error and error estimates together, for the first four
eigenvalues, and in
Figures~\ref{fig:rel_triup} we plot the corresponding
values of the effectivity quotient.
\begin{quote}
  For problems in which the exact eigenvalues are not known, we should
  list our most accurate approximations, probably together with an
  idea of how many digits can be trusted. \hfill Jeff
\end{quote}
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_triup.eps}
\end{center}
\caption{\label{fig:error_triup} Errors and error estimates. Triangle
  with hole.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_triup.eps}
\end{center}
\caption{\label{fig:rel_triup} Effectivity index. Triangle with hole.}
\end{figure}


\subsection{Square Domain with Discontinuous Reaction Term}\label{Dauge1}
For this series of problems we take $\Omega=(-1,1)^2$,
$\nabla\psi\cdot\mb{n}=0$ on $\partial\Omega$, and
$\cL\,\psi=-\Delta \psi+\kappa V_{MD}\cdot\psi$, where $V_{MD}$ is the
characteristic function of the touching squares labelled $\cM_1$ in
Figure~\ref{figMonique}.  We consider several values of the constant
parameter $\kappa>0$.  It is straightforward to see that the
corresponding bilinear form is an inner-product in this case (no zero
eigenvalues), and that all eigenfunctions are at least in $H^2$.
\begin{quote}
  Luka, you mentioned some specific series of $\kappa$s, either going
  to zero or infinity.  Could you put what you have in mind here,
  together with an explanation of significance (you mentioned
  something about ``tunnelling'')?

  The experiments here will have to be re-run, because they were
  probably for a problem with discontinuous diffusion instead. \hfill Jeff
\end{quote} 
%This example was originally proposed and
%solved as a test example for an eigenvalue problem in electromagnetism by
%M. Dauge in \cite{DaugeW}. In its original formulation the problem is much more challenging, since
%the jumps are contained in the second order term, cf. \cite{DaugeW}. A similar problem --- having jumps in the second order term --- has also been
%studied as an interesting example in the context of ill-posed boundary value problems by Knyazev and Widlund in \cite{Knyazev2003}. There,
%an extensive regularity theory for such problems is presented as well.


\begin{figure}[h!]
\begin{center}
%\includegraphics[width=8.5cm]{2DomE.eps}
\begin{picture}(0,0)%
\includegraphics{Dauge.eps}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(2724,2724)(1339,-523)
\put(1850,1490){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_2$}%
}}}}
\put(3200,140){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_2$}%
}}}}
\put(3200,1490){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_1$}%
}}}}
\put(1850,140){\makebox(0,0)[lb]{\smash{{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{$\mathcal{M}_1$}%
}}}}
\end{picture}%
\end{center}
\caption{\label{figMonique} A modification of the touching squares
  example of M. Dauge.}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_neu_jumps_0.5.eps}
\end{center}
\caption{\label{fig:error_neu_jumps_0.5} Errors and error estimates. 
  Discontinuous reaction term, $\kappa=0.5$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_neu_jumps_0.5.eps}
\end{center}
\caption{\label{fig:rel_neu_jumps_0.5} Effectivity
  index. Discontinuous reaction term, $\kappa=0.5$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_neu_jumps_eig1.eps}
\end{center}
\caption{\label{fig:error_neu_jumps_eig1} Errors and error estimates. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_neu_jumps_eig1.eps}
\end{center}
\caption{\label{fig:rel_neu_jumps_eig1} Effectivity
  index. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}


Then we choose $\kappa=0.1$ and we consider the first eigenvalue different from zero.
In Figure~\ref{fig:error_neu_jumps_eig1} we plot the error $\frac{\hat\lambda_2-\lambda_2}{\hat\lambda_2}$ and the residuals ${\hat\lambda_2}^{-1}\varepsilon_2^2$ using $hp-$adaptivity, also in Figure~\ref{fig:rel_neu_jumps_eig1} we plot the correspondent values of the effectivity constant $C$.

It is interesting to compare the previous plots with the next ones, where we consider the first three eigenvalues different from 0, namely $\lambda_j$, $j=2,3,4$.
In Figure~\ref{fig:error_neu_jumps_0.1} we plot the error and the residuals and in Figure~\ref{fig:rel_neu_jumps_0.1} we plot the correspondent values of the effectivity constant $C$.

As can be seen the convergence is much slower and the reason for that can be found looking at Figure~\ref{fig:error_split_neu_jumps_0.1} where we plot the errors for each eigenvalue separately.
As can be seen it is the third eigenvalue that is the slowest and the one to slow down the overall convergence. This seems to suggest that the third eigenvalue is much less regular than the other two.
In Figure~\ref{fig:eig2},~\ref{fig:eig3} and~\ref{fig:eig4} we plot the counter plots for the three considered eigenfunctions.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_neu_jumps_0.1.eps}
\end{center}
\caption{\label{fig:error_split_neu_jumps_0.1} Errors from each
  eigenvlaue. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0002.eps}
\end{center}
\caption{\label{fig:eig2} Second eigenfunction. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0003.eps}
\end{center}
\caption{\label{fig:eig3} Third eigenfunction. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.3]{visit0004.eps}
\end{center}
\caption{\label{fig:eig4} Fourth eigenfunction. Discontinuous reaction term, $\kappa=0.1$.}
\end{figure}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Square Domain with Discontinuous Diffusion Term}
Using the domain $\Omega=(-1,1)^2$, partitioned into regions $\cM_1$
and $\cM_2$ as in Figure~\ref{figMonique}, and homogeneous Dirichlet
conditions $\psi=0$ on $\partial\Omega$, we consider the operator
$\cL=-a\Delta$, where $a=1$ in $\cM_2$ and $a=?$ in $\cM_1$.  Such
problems can have nearly arbitrarily bad singularites at the origin
depending on the relative sizes of $a$ in the two subdomains---see,
for example,~\cite{Kellogg1975} or a computational look at one of the
relevant (to our problem) examples of that paper in~\cite[Example
5.3]{Morin2000}.

\subsection{Suare Domain with a Slit}
For this problem, $\cL=-\Delta$ and $\Omega=(0,1)^2\setminus S$, where
$S=\{(x,1/2):\,1/2<x<1\}$; this is pictured in
Figure~\ref{fig:domains}, with $S$ as the dashed segment.  Homogeneous
Neumann
conditions are imposed on the top and bottom of $S$, and homogeneous
Dirichlet
condtions are imposed on the rest of the boundary.

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_crack2.eps}
\end{center}
\caption{\label{fig:lap_err_crack2_hp} Errors and error
  estimates. Slit square. Second eigenvalue only.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_crack2.eps}
\end{center}
\caption{\label{fig:lap_rel_crack2_hp} Effectivity index. Slit square. Second eigenvalue only.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_crack.eps}
\end{center}
\caption{\label{fig:lap_err_crack_hp} Errors and error estimates. Slit
  square. First four eigenvalues.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{rel_crack2.eps}
\end{center}
\caption{\label{fig:lap_rel_crack_hp} Effectivity index. Slit
  square. First four eigenvalues.}
\end{figure}

\begin{figure}[h!]
\begin{center}
\includegraphics[scale=0.6]{error_split_crack.eps}
\end{center}
\caption{\label{fig:lap_err_split_crack_hp} Errors from each eigenvlaue. Slit
  square.}
\end{figure}


We start considering the second eigenvalue, which seems to be highly irregular.
In Figure~\ref{fig:lap_err_crack2_hp} we plot the error $\frac{\hat\lambda_2-\lambda_2}{\hat\lambda_2}$ and the residuals ${\hat\lambda_2}^{-1}\varepsilon_2^2$ using $hp-$adaptivity. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_crack2_hp} we plot the values of the effectivity constant $C$ for the simulations already considered in Figure~\ref{fig:lap_err_crack2_hp}, again the values of $C$ are very well clustered, as predicted by the theory. Then, in Figure~\ref{fig:lap_err_crack_hp} we plot the error $\sum_{i=1}^4\frac{\hat\lambda_i-\lambda_i}{\hat\lambda_i}$ and the residuals $\sum_{i=1}^4{\hat\lambda_i}^{-1}\varepsilon_i^2$ using $hp-$adaptivity. In also this case the convergence is exponential.
In Figure~\ref{fig:lap_rel_crack_hp} we plot the values of the effectivity constant $C$.
Comparing  Figure~\ref{fig:lap_err_crack2_hp} with Figure~\ref{fig:lap_err_crack_hp} it is clear that the convergence is very similar, but then looking at Figure~\ref{fig:lap_err_split_crack_hp}, where the plots of the error for each eigenvalue are reported, it is also clear that the error for the second eigenvalue is dominant compared to the errors for the other eigenvalues, which are smoother and converge faster.



\subsection{Eigenvalues on a Slit Disk}
For this problem, $\cL=-\Delta$ and
$\Omega={(x,y):\,x^2+y^2<1}\setminus S$, where $S=\{(x,0):\,0<x<1\}$;
this is pictured in Figure~\ref{fig:domains}, with $S$ as the dashed
segment.  Homogeneous Neumann conditions are imposed on the bottom of
$S$, and homogeneous Dirichlet condtions are imposed on the top of $S$
and the rest of the boundary. In this case, the eigenvalues and
eigenfunctions are known explicitly.  Let $\nu_k=(2k-3)/4$ for
$k\in\NN$, and $z_{km}$ be the $m^{th}$ positive root of the
first-kind Bessel function $J_{\nu_k}$.  It is straightforward to
verify that, up to renormalization of eigenfunctions, the eigenpairs
can be indexed by
\begin{align*}
\lambda_{km}=z_{km}^2\quad,\quad
\psi_{km}=J_{\nu_k}(z_{km}r)\sin(\nu_k \theta)\quad,\quad k,m\in\NN~.
\end{align*}
We see that
$\psi_{km}\sim \sin(\nu_k
\theta)\left(\frac{z_{km}r}{2}\right)^{\nu_k}$ as $r\to 0$, so
singularities of types $r^{\nu_k}$ occur infinitely many times
in the spectrum.  The strongest of these singularities is of type
$r^{1/4}$, and it occurs in the eigenfunctions associated
with the first (smallest) and sixth eigenvalues, for example.
The eigenvalues can, in principle, be computed to abitrary precision
by using a computer algebra system, and we give
the smallest six of them below, accurate to all $30$ digits
shown---up to rounding in the last digit.
\begin{align*}
\begin{array}{|ccc|}
\hline
k&m&\lambda_{km}\\\hline
1&1&7.73333653346596686390263803337\\
2&1&12.1871394680951290047505723560\\
3&1&17.3507761313694859586686502730\\
4&1&23.1993865387331719385298116070\\
5&1&29.7145342842106938075714690649\\
1&2&34.8825215790904790430911907100\\\hline
\end{array}
\end{align*}
%%% 6&1&36.8818928841180487579063517659


